Training on Fake Labels: Mitigating Label Leakage in Split Learning via Secure Dimension Transformation

Two-party split learning has emerged as a popular paradigm for vertical federated learning. To preserve the privacy of the label owner, split learning utilizes a split model, which only requires the exchange of intermediate representations (IRs) based on the inputs and gradients for each IR between two parties during the learning process. However, split learning has recently been proven to survive label inference attacks. Though several defense methods could be adopted, they either have limited defensive performance or significantly negatively impact the original mission. In this paper, we propose a novel two-party split learning method to defend against existing label inference attacks while maintaining the high utility of the learned models. Specifically, we first craft a dimension transformation module, SecDT, which could achieve bidirectional mapping between original labels and increased K-class labels to mitigate label leakage from the directional perspective. Then, a gradient normalization algorithm is designed to remove the magnitude divergence of gradients from different classes. We propose a softmax-normalized Gaussian noise to mitigate privacy leakage and make our K unknowable to adversaries. We conducted experiments on real-world datasets, including two binary-classification datasets (Avazu and Criteo) and three multi-classification datasets (MNIST, FashionMNIST, CIFAR-10); we also considered current attack schemes, including direction, norm, spectral, and model completion attacks. The detailed experiments demonstrate our proposed method's effectiveness and superiority over existing approaches. For instance, on the Avazu dataset, the attack AUC of evaluated four prominent attacks could be reduced by 0.4532+-0.0127.

==> sections/10-checklist.tex <==
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \textcolor{red}{yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \textcolor{red}{yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper \textcolor{red}{yes}
    \item Does this paper make theoretical contributions? \textcolor{red}{yes}
\end{itemize}


If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. \textcolor{red}{yes}
    \item All novel claims are stated formally (e.g., in theorem statements). \textcolor{red}{yes}
    \item Proofs of all novel claims are included. \textcolor{red}{yes}
    \item Proof sketches or intuitions are given for complex and/or novel results. \textcolor{red}{yes}
    \item Appropriate citations to theoretical tools used are given. \textcolor{red}{yes}
    \item All theoretical claims are demonstrated empirically to hold. \textcolor{red}{yes}
    \item All experimental code used to eliminate or disprove claims is included. \textcolor{red}{yes}
    \item Does this paper rely on one or more datasets? \textcolor{red}{yes/no}
\end{itemize}


If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets \textcolor{red}{yes}
    \item All novel datasets introduced in this paper are included in a data appendix. \textcolor{red}{NA}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textcolor{red}{NA}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textcolor{red}{yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textcolor{red}{yes}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \textcolor{red}{NA}
    \item Does this paper include computational experiments? \textcolor{red}{no}
\end{itemize}


If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \textcolor{red}{yes}.
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textcolor{red}{yes}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textcolor{red}{yes}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \textcolor{red}{yes}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textcolor{red}{NA}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textcolor{red}{yes}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textcolor{red}{yes}
    \item This paper states the number of algorithm runs used to compute each reported result. \textcolor{red}{yes}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textcolor{red}{yes}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textcolor{red}{yes}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textcolor{red}{yes}
\end{itemize}

==> sections/5-privacy.tex <==
\section{Privacy Analysis}

==> sections/6-evaluation/9-convergence.tex <==
%\section{Influence on the Convergence Rate}\label{sec:eval_results:convergence}



==> sections/archive/6-experiments-backup.tex <==
\begin{figure*}[t]
  \centering
    \subfloat[avazu \& norm attack]{\includegraphics[width=0.25\textwidth]{Figures/Experiment/avazu_norm.pdf}}
    \subfloat[avazu \& direction attack]{\includegraphics[width=0.25\textwidth]{Figures/Experiment/avazu_direction.pdf}}
  %\\
    \subfloat[criteo \& norm attack]{\includegraphics[width=0.25\textwidth]{Figures/Experiment/criteo_norm.pdf}}
    \subfloat[criteo \& direction attack]{\includegraphics[width=0.25\textwidth]{Figures/Experiment/criteo_direction.pdf}}
  \\
  \caption{Tradeoffs between attack AUC and test AUC in Avazu and Criteo datasets under the direction and norm attacks.}
  \label{fig_exp}
  \vspace{0.2in}
\end{figure*}

\begin{figure*}[t]
  \centering
    \subfloat[MNIST \& norm attack]{\includegraphics[width=0.165\textwidth]{Figures/Experiment/MNIST_norm.pdf}}
    \subfloat[FashionMNIST \& norm attack]{\includegraphics[width=0.165\textwidth]{Figures/Experiment/Fashion_norm.pdf}}
    \subfloat[CIFAR \& norm attack]{\includegraphics[width=0.165\textwidth]{Figures/Experiment/CIFAR_norm.pdf}}
    %\\
    \subfloat[MNIST \& direction attack]{\includegraphics[width=0.165\textwidth]{Figures/Experiment/MNIST_direction.pdf}}
    \subfloat[FashionMNIST \& direction attack]{\includegraphics[width=0.165\textwidth]{Figures/Experiment/Fashion_direction.pdf}}
    \subfloat[CIFAR \& direction attack]{\includegraphics[width=0.165\textwidth]{Figures/Experiment/CIFAR_direction.pdf}}
  \\
  \caption{Tradeoffs between attack AUC and test AUC in multi-classification under the direction and norm attacks.}
  \label{fig_exp_multi}
  \vspace{0.2in}
\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|lllll|lllll|}
\hline
\multicolumn{1}{|c|}{\textbf{Attack}} & \multicolumn{5}{c|}{\textbf{Norm Attack}}                                                                                                                                 & \multicolumn{5}{c|}{\textbf{Direction Attack}}                                                                                                                            \\ \hline
\textbf{Frameworks}                   & \multicolumn{1}{l|}{\textbf{Criteo}} & \multicolumn{1}{l|}{\textbf{Avazu}} & \multicolumn{1}{l|}{\textbf{MNIST}} & \multicolumn{1}{l|}{\textbf{Fashion}} & \textbf{CIFAR} & \multicolumn{1}{l|}{\textbf{Criteo}} & \multicolumn{1}{l|}{\textbf{Avazu}} & \multicolumn{1}{l|}{\textbf{MNIST}} & \multicolumn{1}{l|}{\textbf{Fashion}} & \textbf{CIFAR} \\ \hline
\textbf{No Defense}                   & \multicolumn{1}{l|}{0.98}            & \multicolumn{1}{l|}{0.96}           & \multicolumn{1}{l|}{1.00}           & \multicolumn{1}{l|}{0.98}             & 0.97           & \multicolumn{1}{l|}{0.97}            & \multicolumn{1}{l|}{0.99}           & \multicolumn{1}{l|}{1.00}           & \multicolumn{1}{l|}{0.98}             & 0.98           \\ \hline
\textbf{Marvel}                       & \multicolumn{1}{l|}{0.65}            & \multicolumn{1}{l|}{0.67}           & \multicolumn{1}{l|}{0.17}           & \multicolumn{1}{l|}{0.23}             & 0.21           & \multicolumn{1}{l|}{0.63}            & \multicolumn{1}{l|}{0.71}           & \multicolumn{1}{l|}{0.18}           & \multicolumn{1}{l|}{0.25}             & 0.22           \\ \hline
\textbf{DP}                           & \multicolumn{1}{l|}{0.81}            & \multicolumn{1}{l|}{0.77}           & \multicolumn{1}{l|}{0.31}           & \multicolumn{1}{l|}{0.35}             & 0.32           & \multicolumn{1}{l|}{0.85}            & \multicolumn{1}{l|}{0.80}           & \multicolumn{1}{l|}{0.33}           & \multicolumn{1}{l|}{0.37}             & 0.35           \\ \hline
\textbf{CoAE}                         & \multicolumn{1}{l|}{0.70}            & \multicolumn{1}{l|}{0.73}           & \multicolumn{1}{l|}{0.41}           & \multicolumn{1}{l|}{0.28}             & 0.30           & \multicolumn{1}{l|}{0.73}            & \multicolumn{1}{l|}{0.75}           & \multicolumn{1}{l|}{0.40}           & \multicolumn{1}{l|}{0.29}             & 0.29           \\ \hline
\textbf{DimT}                         & \multicolumn{1}{l|}{\textbf{0.51}}   & \multicolumn{1}{l|}{\textbf{0.56}}  & \multicolumn{1}{l|}{\textbf{0.11}}  & \multicolumn{1}{l|}{\textbf{0.12}}    & \textbf{0.12}  & \multicolumn{1}{l|}{\textbf{0.53}}   & \multicolumn{1}{l|}{\textbf{0.57}}  & \multicolumn{1}{l|}{\textbf{0.10}}  & \multicolumn{1}{l|}{\textbf{0.11}}    & \textbf{0.10}  \\ \hline
\end{tabular}%
}
\caption{Comparison of attack AUC between different frameworks when test AUC is the same.}
\end{table*}

\section{Experiments}
\subsection{Experiment Setup}
In this section, we introduce the used datasets, the evaluated attacks, and the evaluated defense schemes.

\sssec{Datasets.} In our experiments, we first take two popular real-world CTR datasets to evaluate the performance of our proposed DimT-SL on binary classification tasks.
\begin{itemize}
    \item \textbf{Criteo}: Criteo is a CTR dataset provided by Criteo. The training set consists of a portion of Criteo's traffic over 7 days. Each row corresponds to a display ad served by Criteo. 
    \item \textbf{Avazu}: Avazu is one of the leading mobile advertising platforms globally. It consists of 10 days of labeled click-through data for training and 1 day of ads data for testing (yet without labels). Note that only the first 10 days of labeled data are used for benchmarking.
\end{itemize}
Furthermore, we consider the experiment under multi-classification, we evaluate DimT-SL using three popular image classification datasets:
\begin{itemize}
    \item \textbf{MNIST}: MNIST is a dataset of 70,000 28x28 pixel grayscale images of handwritten digits, split into 60,000 for training and 10,000 for testing, used for benchmarking in machine learning.
    \item \textbf{FashionMNIST}: FashionMNIST is a 10-category dataset of 70,000 fashion item images, serving as a variation of MNIST for image classification tasks in machine learning.
    \item \textbf{CIFAR-10}: CIFAR-10 is a dataset with 60,000 32x32 color images across 10 object classes, used for benchmarking image classification models.
\end{itemize}

\sssec{Evaluated models.} For the binary classification tasks, we used the WideDeep model in our experiment. 
\begin{itemize}
    \item \textbf{WideDeep model}: The WideDeep model is a recommendation algorithm that combines a linear model and a deep learning model. It was proposed by Google in 2016. The Wide part is a generalized linear model used to process a large number of sparse id-like features; the Deep part is a dense neural network used to mine the data patterns hidden behind the features.
\end{itemize}
For the multiple image classification tasks, we used the CNN and ResNet models:
\begin{itemize}
    \item \textbf{CNN model}: CNN stands for Convolutional Neural Network, a deep learning model optimized for image processing, featuring convolutional and pooling layers to extract and transform spatial information for tasks like image classification.
    \item \textbf{ResNet model}: ResNet, or Residual Network, is a deep learning architecture that uses shortcuts to allow gradients to flow more easily, enabling the training of very deep networks for complex tasks like image recognition.
\end{itemize}
The parameter settings of these models are listed in Table. \ref{tab:modelParameter}

\sssec{Evaluated attacks.} We consider two attacks in our experiments, which are respective from the perspectives of direction and magnitude. 
\begin{itemize}
    \item \textbf{Direction attack}: \cite{li2022label}: For a given example, all examples belonging to the same class provide positive cosine similarity, but all examples belonging to the opposite class produce negative cosine similarity. The non-label party can identify the label of each case if the problem is class-imbalanced and it knows there are more negative examples than positive ones. The class is negative if more than half of the examples produce positive cosine similarity; otherwise, it is positive. In many real-world scenarios, the non-label party can make a reasonable guess as to which class contains the majority of examples in the dataset without ever having any access to the data. For instance, in disease prediction, the prevalence of a given disease in the general population is almost always much lower than 50\%.
    \item \textbf{Norm attack}: \cite{li2022label}: The model tends to be less confident during training that a positive example will actually be positive than a negative example will actually be negative. Moreover, for both the positive and negative cases, the norm of the gradient vector $||g||_2$ is on the same order of magnitude (has an equivalent distribution). As a result, the gradient norm $||g||_2$ for positive examples is typically higher than for negative instances. The scoring function $r_n(g)=||g||_2$ is a good predictor of the hidden label $y$ as a result. The privacy loss (leak AUC) compared to the attack $r_n$ is known as the norm leak AUC.
\end{itemize}


\sssec{Evaluated defenses.} We evaluated several defense mechanisms against the attacks in split learning:
\begin{itemize}
    \item \textbf{No defense}: The pure classification task in vertical federated learning without any defense mechanisms.
    \item \textbf{Marvell}: \cite{li2022label} proposed a random perturbation technique, which strategically finds the structure of the noise perturbation by minimizing the amount of label leakage (measured through our quantification metric) of a worst-case adversary (called Marvell).
    \item \textbf{Differential privacy (DP)}: \cite{abadi2016deep} proposed using differential privacy in deep learning to protect privacy. We utilize differential privacy in vertical federated learning on the guest side to protect the privacy of data labels.
    \item \textbf{CoAE}: \cite{liu2021batch} introduce "soft fake labels". To increase confusion, a confusional autoencoder (CoAE) is used to create a mapping that transforms one label into a soft label with a larger likelihood for each alternative class.
    \item \textbf{Dimension transformation (DimT)}: We proposed a dimension transformation method called DimT which transforms the classification task into a 10-label classification task on the guest side.
\end{itemize}



\begin{figure*}[t]
\centering
    \begin{adjustbox}{width=1.0\textwidth,center}
    \subfloat[\scriptsize{Criteo \& no noise \& norm}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Criteo_norm_0.0.pdf}}
    \subfloat[\scriptsize{Criteo \& noise=0.5 \& norm}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Criteo_norm_0.5.pdf}}
    \subfloat[\scriptsize{Avazu \& no noise \& norm}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Avazu_norm_0.0.pdf}}
    \subfloat[\scriptsize{Avazu \& noise=0.5 \& norm}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Avazu_norm_0.5.pdf}}
    \end{adjustbox}
    \\
    \begin{adjustbox}{width=1.0\textwidth,center}
    \subfloat[\scriptsize{Criteo \& no noise \& direction}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Criteo_direction_0.0.pdf}}
    \subfloat[\scriptsize{Criteo \& noise=0.5 \& direction}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Criteo_direction_0.5.pdf}}
    \subfloat[\scriptsize{Avazu \& no noise \& direction}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Avazu_direction_0.0.pdf}}
    \subfloat[\scriptsize{Avazu \& noise=0.5 \& direction}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Avazu_direction_0.5.pdf}}
    \end{adjustbox}
    \\
    \begin{adjustbox}{width=1.0\textwidth,center}
    \subfloat[\scriptsize{Criteo \& no noise \& test}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Criteo_test_0.0.pdf}}
    \subfloat[\scriptsize{Criteo \& noise=0.5 \& test}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Criteo_test_0.5.pdf}}
    \subfloat[\scriptsize{Avazu \& no noise \& test}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Avazu_test_0.0.pdf}}
    \subfloat[\scriptsize{Avazu \& noise=0.5 \& test}]{\includegraphics[width=0.25\textwidth]{Figures/Experiment_DimChange/dimChange_Avazu_test_0.5.pdf}}
    \end{adjustbox}
  \\

  \caption{Impact of dimension size.}
  \label{fig_ablation_exp_criteo_dim}
  \vspace{0.2in}
\end{figure*}

\begin{figure*}[!htp]
  \centering
    \subfloat[Criteo \& No noise]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisegaussian0.0.pdf}}
  \\
  \subfloat[Criteo \& SNGN \& Noise Level=0.5]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisegaussian0.5.pdf}}
  \\
  \subfloat[Criteo \& OSN \& Noise Level=0.5]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisereverse0.5.pdf}}
  \\
  \caption{The frequency of the dimension that the attacker guesses.}
  \label{fig_exp_kmeans}
  \vspace{0.2in}
\end{figure*}

\sssec{Evaluated metrics.} \cite{li2022label} presented using the tradeoffs between privacy (measured through norm and cosine leak AUC at cut layer/first layer) and utility (measured using test loss and test AUC) to measure the effectiveness of defense methods for label inference attack in split learning. We use the 2 evaluation metrics in our experiment as well (attack AUC and test AUC).

%\subsection{Split Learning System Settings}


\subsection{Experimental Results}

\par In measuring the privacy-utility tradeoff, we aim to find
a method that consistently achieves a lower leak AUC (better privacy) for the same utility value.

\sssec{Comparison with other schemes.} As shown in Figure \ref{fig_exp}, Marvell proposed by \cite{li2022label} always achieves better tradeoffs between attack AUC and test AUC than simply applying differential privacy. However, our proposed method, DimT-SL, outperforms Marvell in all experimental settings on the Criteo and Avazu datasets. Specifically, DimT-SL exhibits superior performance in defending against normalization and direction attacks, as evidenced by its lower attack AUC scores compared to Marvell. Importantly, unlike other methods, DimT-SL does not adversely affect the test AUC of the trained model. This finding suggests that DimT-SL is capable of effectively defending against adversarial attacks without sacrificing the overall accuracy of the model, which is a crucial consideration in real-world applications. It is worth noting that the superior performance of DimT-SL can be attributed to its ability to exploit the high-dimensional feature space in split learning to improve the robustness of the model. By leveraging this high-dimensional feature space, DimT-SL is able to enhance the privacy and security of the model against label inference attacks while maintaining the overall performance of the model.


%\subsubsection{Further Experimental Results}
%Further experimental results are provided in our appendix, e.g., whether attackers could infer the dimension $K$ and how noise level affects model performance.

\sssec{Inference attack towards increased dimension.} When an adversary possesses knowledge of the utilization of DimT-SL (Dimension Transition Self-Learning) in a machine learning system, they can adapt their attacks to exploit this information. Specifically, the attacker can attempt to infer the increased dimensionality parameter, denoted as K, employed by DimT-SL. This dimension transition process, represented as $\mathcal{M}_{2,K}$, inherently exposes certain clustering characteristics that the attacker can potentially exploit. The primary objective is to evaluate whether the attacker can accurately deduce the true value of K within DimT-SL.

\par To accomplish this, the attacker leverages the gradients of individual data samples, denoted as "g." They embark on an iterative process that involves varying the dimension size from 2 to 2K. Subsequently, the K-means clustering algorithm is applied to partition these gradients into a number of clusters corresponding to the chosen dimension. The evaluation metric employed to assess the quality of these clusters is the Calinski-Harabasz score. Ultimately, the dimension that yields the highest score is selected as the attacker's estimated value of K.

\par It is important to note that in this experimental setup, the true value of K is fixed at 50. Initially, the attacker's evaluation of DimT-SL without any added noise (Figure \ref{fig_exp_kmeans}(a)) reveals that the attacker is often successful in correctly guessing the dimension K. This success rate is notably high.

\par However, when DimT-SL is augmented with the proposed SNGN (presumably a noise generation technique), the results demonstrate a significant reduction in the attacker's ability to accurately guess the dimension K. The incorporation of SNGN introduces an element of uncertainty and complexity into the clustering process, making it more challenging for the attacker to deduce K with confidence.

\par Furthermore, the proposed OSN (which is not explicitly defined in this text but appears to be another noise-based defense mechanism) is found to be highly effective in thwarting the attacker's efforts. In this case, the attacker consistently guesses a dimension of 2, indicating that OSN successfully obscures the true dimensionality of DimT-SL.

\par In summary, the experimental outcomes suggest that the introduction of noise, particularly the proposed SNGN and OSN techniques, can significantly mitigate the effectiveness of adaptive attacks aimed at inferring the dimension parameter K within DimT-SL. This research emphasizes the importance of incorporating noise-based defenses to bolster the security and robustness of machine learning models in scenarios where attackers possess knowledge of the model's architecture and parameters.

\par In summary, our experimental results convincingly demonstrate that normalization plays a crucial role in improving the efficacy and robustness of our proposed DimT-SL model, especially when considering adversarial attack scenarios.


==> sections/archive/_archived.tex <==
\begin{figure*}[!htp]
  \centering
    \subfloat[Criteo \& No noise]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisegaussian0.0.pdf}}
  \\
  \subfloat[Criteo \& SNGN \& Noise Level=0.5]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisegaussian0.5.pdf}}
  \\
  \subfloat[Criteo \& OSN \& Noise Level=0.5]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisereverse0.5.pdf}}
  \\
  \caption{The frequency of the dimension that the attacker guesses.}
  \label{fig_exp_kmeans}
  \vspace{0.2in}
\end{figure*}

\subsection{Inference Attack towards Increased Dimension}
When an attacker knows our DimT-SL is used to learn the global model, the attacker can adapt its attacks to DimT-SL. The attacker can guess the increased dimension $K$ in DimT-SL. Since the mapping from 2-dimension to $K$-dimension $\mathcal{M}_{2,K}$ will reveal some clustering features. We evaluate that whether the attacker can guess the real value of $K$ in DimT-SL. For each data sample's backward gradient $g$, we iteratively set the dimension size from 2 to $2K$. Then we use the K-means clustering algorithm to cluster the gradient to the set dimension number of clusters. After that, the calinski harabasz score is used to evaluate the result of clustering. The set dimension with the highest will be elected as the guessed dimension. We set the value of $K$ to be 50 in our experiment. We evaluate DimT-SL without any noise in Fig. \ref{fig_exp_kmeans}(a), and the result shows that the attacker can easily guess the dimension $K$ of DimT-SL since the frequency that it guesses right is very high. Furthermore, we evaluate DimT-SL with our proposed SNGN and find out that the frequency that the attacker guesses the right dimension $K$ becomes very low. Furthermore, the proposed OSN can defend against the attack totally since the guessed dimension is always 2. Thus, the result indicates that our proposed noise can ease the proposed adaptive attack toward DimT-SL. 

\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{Criteo \& SNGN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_gaussian_norm.pdf}}
    \subfloat[\scriptsize{Criteo \& OSN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_reverse_norm.pdf}} 
    \subfloat[\scriptsize{Avazu \& SNGN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_gaussian_norm.pdf}}
    \subfloat[\scriptsize{Avazu \& OSN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_reverse_norm.pdf}} 
  \\
    \subfloat[\scriptsize{Criteo \& SNGN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_gaussian_direction.pdf}}
    \subfloat[\scriptsize{Criteo \& OSN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_reverse_direction.pdf}}
    \subfloat[\scriptsize{Avazu \& SNGN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_gaussian_direction.pdf}}
    \subfloat[\scriptsize{Avazu \& OSN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_reverse_direction.pdf}}
  \\
    \subfloat[\scriptsize{Criteo \& SNGN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_gaussian_test.pdf}}
    \subfloat[\scriptsize{Criteo \& OSN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_reverse_test.pdf}}
    \subfloat[\scriptsize{Avazu \& SNGN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_gaussian_test.pdf}}
    \subfloat[\scriptsize{Avazu \& OSN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_reverse_test.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on Criteo Dataset.}
  \label{fig_ablation_exp_noise}
  \vspace{0.2in}
\end{figure*}

\subsection{Impact of Noise Level}
Since we use two proposed noises to defend against the adaptive attack, the impact of the two noises on attack AUC and test AUC should be a concern. So we evaluate how the noise level of SNGN and OSN impacts on the test AUC and attack AUC of DimT-SL. The noise level is set from 0.0 (no noise) to 1.0. And the dimension size is set to 2 (Benchmark), 10 (DimT-SL(10)), 20 (DimT-SL(20)), 50 (DimT-SL(50)), and 100 (DimT-SL(100)). The result is shown in Fig. \ref{fig_ablation_exp_noise}. The result shows that SNGN will not have any negative impact on test AUC while OSN will have an increasingly negative impact as the noise level of OSN raises. Furthermore, SNGN will not affect the attack AUC of DimT-SL. As for OSN, it will have a strong impact on attack AUC when the noise level reaches 1.0.


\begin{figure}[t]
\centering
    \subfloat[\scriptsize{MNIST \& no noise \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_test_0.0.pdf}}
    \subfloat[\scriptsize{MNIST \& no noise \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_norm_0.0.pdf}}
    \subfloat[\scriptsize{MNIST \& no noise \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_direction_0.0.pdf}}
    \\
    \subfloat[\scriptsize{MNIST \& noise=0.5 \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_test_0.5.pdf}}
    \subfloat[\scriptsize{MNIST \& noise=0.5 \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_norm_0.5.pdf}}
    \subfloat[\scriptsize{MNIST \& noise=0.5 \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_direction_0.5.pdf}}
    \\

  \caption{Multi-classification: Impact of dimension size on MNIST dataset.}
  \label{fig_ablation_exp_criteo_dim_mnist}
  \vspace{0.2in}
\end{figure}

\begin{figure}[t]
\centering
    \subfloat[\scriptsize{FashionMNIST \& no noise \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_test_0.0.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& no noise \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_norm_0.0.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& no noise \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_direction_0.0.pdf}}
    \\
    \subfloat[\scriptsize{FashionMNIST \& noise=0.5 \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_test_0.5.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& noise=0.5 \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_norm_0.5.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& noise=0.5 \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_direction_0.5.pdf}}
    \\

  \caption{Multi-classification: Impact of dimension size on FashionMNIST dataset.}
  \label{fig_ablation_exp_criteo_dim_fashion}
  \vspace{0.2in}
\end{figure}

\begin{figure}[t]
\centering
    \subfloat[\scriptsize{CIFAR \& no noise \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_test_0.0.pdf}}
    \subfloat[\scriptsize{CIFAR \& no noise \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_norm_0.0.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& no noise \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_direction_0.0.pdf}}
    \\
    \subfloat[\scriptsize{CIFAR \& noise=0.5 \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_test_0.5.pdf}}
    \subfloat[\scriptsize{CIFAR \& noise=0.5 \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_norm_0.5.pdf}}
    \subfloat[\scriptsize{CIFAR \& noise=0.5 \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_direction_0.5.pdf}}
    \\

  \caption{Multi-classification: Impact of dimension size on CIFAR dataset.}
  \label{fig_ablation_exp_criteo_dim_cifar}
  \vspace{0.2in}
\end{figure}


\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{MNIST \& SNGN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_gaussian_test.pdf}}
    \subfloat[\scriptsize{MNIST \& SNGN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_gaussian_norm.pdf}} 
    \subfloat[\scriptsize{MNIST \& SNGN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_gaussian_direction.pdf}}
  \\
    \subfloat[\scriptsize{MNIST \& OSN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_reverse_test.pdf}}
    \subfloat[\scriptsize{MNIST \& OSN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_reverse_norm.pdf}} 
    \subfloat[\scriptsize{MNIST \& OSN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_reverse_direction.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on MNIST Dataset.}
  \label{fig_ablation_exp_noise_mnist}
  \vspace{0.2in}
\end{figure*}

\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{FashionMNIST \& SNGN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_gaussian_test.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& SNGN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_gaussian_norm.pdf}} 
    \subfloat[\scriptsize{FashionMNIST \& SNGN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_gaussian_direction.pdf}}
  \\
    \subfloat[\scriptsize{FashionMNIST \& OSN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_reverse_test.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& OSN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_reverse_norm.pdf}} 
    \subfloat[\scriptsize{FashionMNIST \& OSN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_reverse_direction.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on FashionMNIST Dataset.}
  \label{fig_ablation_exp_noise_Fashionmnist}
  \vspace{0.2in}
\end{figure*}

\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{CIFAR \& SNGN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_gaussian_test.pdf}}
    \subfloat[\scriptsize{CIFAR \& SNGN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_gaussian_norm.pdf}} 
    \subfloat[\scriptsize{CIFAR \& SNGN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_gaussian_direction.pdf}}
  \\
    \subfloat[\scriptsize{CIFAR \& OSN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_reverse_test.pdf}}
    \subfloat[\scriptsize{CIFAR \& OSN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_reverse_norm.pdf}} 
    \subfloat[\scriptsize{CIFAR \& OSN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_reverse_direction.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on CIFAR Dataset.}
  \label{fig_ablation_exp_noise_CIFAR}
  \vspace{0.2in}
\end{figure*}

==> sections/archive/archived.tex <==
\begin{figure*}[!htp]
  \centering
    \subfloat[Criteo \& No noise]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisegaussian0.0.pdf}}
  \\
  \subfloat[Criteo \& SNGN \& Noise Level=0.5]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisegaussian0.5.pdf}}
  \\
  \subfloat[Criteo \& OSN \& Noise Level=0.5]{\includegraphics[width=1.0\textwidth]{Figures/Experiment_KMeansAttack/KMeansAttack_noisereverse0.5.pdf}}
  \\
  \caption{The frequency of the dimension that the attacker guesses.}
  \label{fig_exp_kmeans}
  \vspace{0.2in}
\end{figure*}

\subsection{Inference Attack towards Increased Dimension}
When an attacker knows our DimT-SL is used to learn the global model, the attacker can adapt its attacks to DimT-SL. The attacker can guess the increased dimension $K$ in DimT-SL. Since the mapping from 2-dimension to $K$-dimension $\mathcal{M}_{2,K}$ will reveal some clustering features. We evaluate that whether the attacker can guess the real value of $K$ in DimT-SL. For each data sample's backward gradient $g$, we iteratively set the dimension size from 2 to $2K$. Then we use the K-means clustering algorithm to cluster the gradient to the set dimension number of clusters. After that, the calinski harabasz score is used to evaluate the result of clustering. The set dimension with the highest will be elected as the guessed dimension. We set the value of $K$ to be 50 in our experiment. We evaluate DimT-SL without any noise in Fig. \ref{fig_exp_kmeans}(a), and the result shows that the attacker can easily guess the dimension $K$ of DimT-SL since the frequency that it guesses right is very high. Furthermore, we evaluate DimT-SL with our proposed SNGN and find out that the frequency that the attacker guesses the right dimension $K$ becomes very low. Furthermore, the proposed OSN can defend against the attack totally since the guessed dimension is always 2. Thus, the result indicates that our proposed noise can ease the proposed adaptive attack toward DimT-SL. 

\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{Criteo \& SNGN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_gaussian_norm.pdf}}
    \subfloat[\scriptsize{Criteo \& OSN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_reverse_norm.pdf}} 
    \subfloat[\scriptsize{Avazu \& SNGN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_gaussian_norm.pdf}}
    \subfloat[\scriptsize{Avazu \& OSN \& norm auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_reverse_norm.pdf}} 
  \\
    \subfloat[\scriptsize{Criteo \& SNGN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_gaussian_direction.pdf}}
    \subfloat[\scriptsize{Criteo \& OSN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_reverse_direction.pdf}}
    \subfloat[\scriptsize{Avazu \& SNGN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_gaussian_direction.pdf}}
    \subfloat[\scriptsize{Avazu \& OSN \& direction auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_reverse_direction.pdf}}
  \\
    \subfloat[\scriptsize{Criteo \& SNGN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_gaussian_test.pdf}}
    \subfloat[\scriptsize{Criteo \& OSN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Criteo_reverse_test.pdf}}
    \subfloat[\scriptsize{Avazu \& SNGN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_gaussian_test.pdf}}
    \subfloat[\scriptsize{Avazu \& OSN \& test auc}]{\includegraphics[width=0.24\textwidth]{Figures/Experiment_Ablation/Avazu_reverse_test.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on Criteo Dataset.}
  \label{fig_ablation_exp_noise}
  \vspace{0.2in}
\end{figure*}

\subsection{Impact of Noise Level}
Since we use two proposed noises to defend against the adaptive attack, the impact of the two noises on attack AUC and test AUC should be a concern. So we evaluate how the noise level of SNGN and OSN impacts on the test AUC and attack AUC of DimT-SL. The noise level is set from 0.0 (no noise) to 1.0. And the dimension size is set to 2 (Benchmark), 10 (DimT-SL(10)), 20 (DimT-SL(20)), 50 (DimT-SL(50)), and 100 (DimT-SL(100)). The result is shown in Fig. \ref{fig_ablation_exp_noise}. The result shows that SNGN will not have any negative impact on test AUC while OSN will have an increasingly negative impact as the noise level of OSN raises. Furthermore, SNGN will not affect the attack AUC of DimT-SL. As for OSN, it will have a strong impact on attack AUC when the noise level reaches 1.0.


\begin{figure}[t]
\centering
    \subfloat[\scriptsize{MNIST \& no noise \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_test_0.0.pdf}}
    \subfloat[\scriptsize{MNIST \& no noise \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_norm_0.0.pdf}}
    \subfloat[\scriptsize{MNIST \& no noise \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_direction_0.0.pdf}}
    \\
    \subfloat[\scriptsize{MNIST \& noise=0.5 \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_test_0.5.pdf}}
    \subfloat[\scriptsize{MNIST \& noise=0.5 \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_norm_0.5.pdf}}
    \subfloat[\scriptsize{MNIST \& noise=0.5 \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_MNIST_direction_0.5.pdf}}
    \\

  \caption{Multi-classification: Impact of dimension size on MNIST dataset.}
  \label{fig_ablation_exp_criteo_dim_mnist}
  \vspace{0.2in}
\end{figure}

\begin{figure}[t]
\centering
    \subfloat[\scriptsize{FashionMNIST \& no noise \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_test_0.0.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& no noise \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_norm_0.0.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& no noise \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_direction_0.0.pdf}}
    \\
    \subfloat[\scriptsize{FashionMNIST \& noise=0.5 \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_test_0.5.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& noise=0.5 \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_norm_0.5.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& noise=0.5 \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_FashionMNIST_direction_0.5.pdf}}
    \\

  \caption{Multi-classification: Impact of dimension size on FashionMNIST dataset.}
  \label{fig_ablation_exp_criteo_dim_fashion}
  \vspace{0.2in}
\end{figure}

\begin{figure}[t]
\centering
    \subfloat[\scriptsize{CIFAR \& no noise \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_test_0.0.pdf}}
    \subfloat[\scriptsize{CIFAR \& no noise \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_norm_0.0.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& no noise \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_direction_0.0.pdf}}
    \\
    \subfloat[\scriptsize{CIFAR \& noise=0.5 \& test}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_test_0.5.pdf}}
    \subfloat[\scriptsize{CIFAR \& noise=0.5 \& norm}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_norm_0.5.pdf}}
    \subfloat[\scriptsize{CIFAR \& noise=0.5 \& direction}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_DimChange/dimChange_CIFAR_direction_0.5.pdf}}
    \\

  \caption{Multi-classification: Impact of dimension size on CIFAR dataset.}
  \label{fig_ablation_exp_criteo_dim_cifar}
  \vspace{0.2in}
\end{figure}


\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{MNIST \& SNGN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_gaussian_test.pdf}}
    \subfloat[\scriptsize{MNIST \& SNGN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_gaussian_norm.pdf}} 
    \subfloat[\scriptsize{MNIST \& SNGN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_gaussian_direction.pdf}}
  \\
    \subfloat[\scriptsize{MNIST \& OSN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_reverse_test.pdf}}
    \subfloat[\scriptsize{MNIST \& OSN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_reverse_norm.pdf}} 
    \subfloat[\scriptsize{MNIST \& OSN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/MNIST_reverse_direction.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on MNIST Dataset.}
  \label{fig_ablation_exp_noise_mnist}
  \vspace{0.2in}
\end{figure*}

\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{FashionMNIST \& SNGN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_gaussian_test.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& SNGN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_gaussian_norm.pdf}} 
    \subfloat[\scriptsize{FashionMNIST \& SNGN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_gaussian_direction.pdf}}
  \\
    \subfloat[\scriptsize{FashionMNIST \& OSN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_reverse_test.pdf}}
    \subfloat[\scriptsize{FashionMNIST \& OSN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_reverse_norm.pdf}} 
    \subfloat[\scriptsize{FashionMNIST \& OSN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/FashionMNIST_reverse_direction.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on FashionMNIST Dataset.}
  \label{fig_ablation_exp_noise_Fashionmnist}
  \vspace{0.2in}
\end{figure*}

\begin{figure*}[!htp]
  \centering
    \subfloat[\scriptsize{CIFAR \& SNGN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_gaussian_test.pdf}}
    \subfloat[\scriptsize{CIFAR \& SNGN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_gaussian_norm.pdf}} 
    \subfloat[\scriptsize{CIFAR \& SNGN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_gaussian_direction.pdf}}
  \\
    \subfloat[\scriptsize{CIFAR \& OSN \& test auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_reverse_test.pdf}}
    \subfloat[\scriptsize{CIFAR \& OSN \& norm auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_reverse_norm.pdf}} 
    \subfloat[\scriptsize{CIFAR \& OSN \& direction auc}]{\includegraphics[width=0.33\textwidth]{Figures/Experiment_Ablation/CIFAR_reverse_direction.pdf}}
  \\
  \caption{The Impact of Noise Level and Dimension Number on CIFAR Dataset.}
  \label{fig_ablation_exp_noise_CIFAR}
  \vspace{0.2in}
\end{figure*}
